On Spectral Analysis of the Internet Delay Space and Detecting Anomalous Routing Paths

Latency is one of the most critical performance metrics for a wide range of applications. Therefore, it is important to understand the underlying mechanisms that give rise to the observed latency values and diagnose the ones that are unexpectedly high. In this paper, we study the Internet delay space via robust principal component analysis (RPCA). Using RPCA, we show that the delay space, i.e. the matrix of measured round trip times between end hosts, can be decomposed into two components - the expected latency between end hosts with respect to the current state of the Internet and the inflation on the paths between the end hosts. Using this decomposition, first we study the well-known low-dimensionality phenomena of the delay space and ask what properties of the end hosts define the dimensions. Second, using the decomposition, we develop a filtering method to detect the paths which experience unexpected latencies and identify routing anomalies. We show that our filter successfully identifies an anomalous route even when its observed latency is not obviously high in magnitude.

==> ack.tex <==

We thank Kc Ng from Akamai Technologies for their feedback and insightful discussions.

==> evaluation.tex <==
We evaluate our method in terms of precision and recall
and resiliency to missing and arbitrarily large data. We 
evaluate our technique in comparison with two other widely 
used methods 2$\sigma$-event detection and regular PCA. 

2$\sigma$-event detection …
 
PCA is a widely used anomaly detection technique. 
As discussed in Section~\ref{sec: } there are significant differences
between RPCA and PCA, i.e. …



\subsection{Precision and Recall}

Labeling the entries: 
It is infeasible to go through 3760(47$\times$80) routing paths manually. In the first step, we aim to follow the 
We follow the following procedure



\subsection{Resiliency to Missing and Arbitrarily Large Values}



Geo RTT based techniques would not really work well. (mention this in the introduction and maybe here again)

